Analysis of the Frequency and Detectability of Objects Resembling Nuclear/Radiological Threats in Commercial Cargo

The threat of smuggled nuclear/radiological weapons and material in commercial containerized cargo remains a significant threat to global security more than a decade after the enactment of laws in the United States and elsewhere mandating interdiction efforts. While significant progress has been made towards deploying passive radiation detection systems in maritime ports, such systems are incapable of detecting shielded threats or even certain scenarios in which material is unshielded. Research efforts towards developing systems for detecting such threats have typically focused on the development of systems that are highly-specific to nuclear/radiological threats and no such systems have been widely deployed. While most existing commercially-available cargo radiography systems are not specifically designed for this interdiction task, if items resembling nuclear/radiological threats are sufficiently rare in cargo radiographs to limit false alarms to an acceptably low frequency, then a smuggling interdiction scheme based on existing technology may be feasible. This analysis characterizes the relevant nuclear and radiological threats that may evade detection by passive monitors, and utilizes a dataset of 122,500 stream-of-commerce cargo container images from a 6 MeV endpoint gamma radiography system to determine the frequency at which objects of similar size and density to such threats occur in containers. It is found that for a broad class of threats, including assembled fission devices, gamma radiography is sufficient to flag threats in this cargo stream at false positive rates of $\lesssim$2%.

==> title.tex <==
Analysis of the Frequency and Detectability of Objects Resembling Nuclear/Radiological Threats in Commercial Cargo
